Classification of Web Phishing Kits for early detection by platform providers

Phishing kits are tools that dark side experts provide to the community of criminal phishers to facilitate the construction of malicious Web sites. As these kits evolve in sophistication, providers of Web-based services need to keep pace with continuous complexity. We present an original classification of a corpus of over 2000 recent phishing kits according to their adopted evasion and obfuscation functions. We carry out an initial deterministic analysis of the source code of the kits to extract the most discriminant features and information about their principal authors. We then integrate this initial classification through supervised machine learning models. Thanks to the ground-truth achieved in the first step, we can demonstrate whether and which machine learning models are able to suitably classify even the kits adopting novel evasion and obfuscation techniques that were unseen during the training phase. We compare different algorithms and evaluate their robustness in the realistic case in which only a small number of phishing kits are available for training. This paper represents an initial but important step to support Web service providers and analysts in improving early detection mechanisms and intelligence operations for the phishing kits that might be installed on their platforms.

==> biographies.tex <==
\textbf{Andrea Venturi} is a PhD student at the International Doctorate School in Information and Communication Technologies (ICT), at the Department of Engineering ``Enzo Ferrari'', University of Modena and Reggio Emilia, Italy. From the same institution, he received the Master's Degree in Computer Engineering \textit{summa cum laude} in 2020 with a thesis on cybersecurity analytics, and the Bachelor's Degree in Computer Science in 2017, with a thesis on data analysis for scalable and distributed networked systems. His research interests are on machine and deep learning applications for cybersecurity.

\textbf{Michele Colajanni} is full professor of computer engineering at the University of Bologna, and affiliated with the Bologna Business School. He graduated in Pisa, and he was with the University of Rome and the University of Modena. His research interests include cybersecurity, scalable architectures for big data management and analytics. He founded the Research Center on Security and Safety and the Cyber Academy for ethical hackers. He has directed courses and masters for universities, ministries, and industries. His scientific production includes more than 250 peer-reviewed articles, and several hundreds of oral presentations in workshops, conferences, and invited lectures.

\textbf{Marco Ramilli} is an international cyber security expert, entrepreneur, writer and white–hat hacker. Ramilli received his PhD on Information Communication Technology. During his PhD he worked for US Government (NIST) where he performed intensive research on Malware evasion techniques and penetration testing methodologies improve USA electronic voting systems. In 2015 he founded Yoroi: an innovative Managed Cyber Security Service Provider developing one of the most amazing cyber security defense centers he has ever experienced. Nowadays, Ramilli leads some of the most talented ethical hackers with a unique mission: to defend private and public organisation on digital space.

\textbf{Giorgio Valenziano Santangelo} is a research fellow at the Department of Engineering "Enzo Ferrari'', University of Modena and Reggio Emilia, Italy. From the same institution, he received the Master's Degree in Computer Engineering in 2020 with a thesis on industrial cybersecurity. His research interests are on cyber attack detection and reverse engineering techniques in industrial contexts.

==> sections/old/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Phishing is an evergreen cyber attack leveraging social engineering methods.
From the initial generic and na\"{i}ve attacks, nowadays phishing is evolving in precision and sophistication with the historical goal of gathering credentials of unaware users~\cite{aleroud2017phishing}. Due to its efficacy, phishing methods are also being used as vectors to spread malware and as a first step to perform other malicious operations~\cite{chiew2018survey}.
From the point of view of an attacker, the creation of a counterfeit copy of a legitimate website and its deployment are laborious and time-consuming phases even because they have to change frequently. \textit{Phishing kits} are created to automate these cumbersome actions. Facilitating the implementation and exploitation of phishing websites expands the number of attackers to even inexperienced criminals to the extent that now they represent one of the most serious menace to cybersecurity~\cite{cova2008there, bijmans2021catching}.

Previous research analyzes specific phishing kits and peculiar functions, but the defenses from this type of attacks deserve a deeper and broader study.
We present the first classification method that groups phishing kits according to their adopted evasion and obfuscation functions.
This analysis represents an opportunity to understand some technical features of the phishing business, and it reveals fundamental information about malicious techniques that security practitioners and hosting providers can use to improve current authorship attribution methodologies and detection mechanisms.

Any classification of phishing kits is challenging because the authors continuously modify the previous versions by introducing novel evasion and obfuscation techniques that complicate the analysis and detection. 
However, we have observed that the most prolific authors introduce new functions but tend to re-use parts of existing material. From a defensive point of view, a similar redundancy represents a key factor because we can provide defenders with a classification of phishing kits based on common malicious functions and characteristics.
%The proposed classification is not immediately oriented *to detect* phishing kits nor to assign them to a specific threat actor, but it is an important support to the anti-phishing ecosystem. 
Our study on the most employed evasion and obfuscation functions adopted in phishing kits can be leveraged by web hosting companies to better comprehend malicious code when it is deployed on their server(s). Moreover, our classification highlights common patterns in the habits of the most popular authors of phishing kits. As phishing is now a mature industry where a small community of expert authors design and implement the phishing kits, it is reasonable to believe that there exist an association between each specific author and his habits in employing evasion and obfuscation functions.
Based on this hypothesis, threat intelligence experts can build author profiles that associate threat actors to the characteristics of their kits. We give an example of a simple author profiling methodology that exploits our classification, and we demonstrate how the most prolific authors tend to maintain the same development habits through time.

The proposed original approach to phishing kit classification consists of multiple phases. The first deterministic analysis builds the ground truth by extracting the usage of the most important evasion and obfuscation functions from the source code of the over 2000 kits. As the deterministic approach is unable to detect unknown techniques, we integrate it with a second probabilistic analysis based on Machine Learning (ML). The idea is to train supervised ML models to recognize evasive and obfuscated kits from structural information and authors' design patterns. The commonly adopted re-utilization allows our classifiers to recognize recurrent patterns of evasive and obfuscated kits. The resulting probabilistic classification can flag even the kits that employ novel evasion and obfuscation techniques that were not considered during training thus addressing main issues of previous deterministic approaches.

%OLD --- The presented classification operates by extracting the most important features from the source code of the phishing kits. Moreover, it investigates whether and which machine learning models are able to classify evasion and obfuscation techniques. We can conclude that most machine learning classifiers guarantee good performance on the identification of evasive and obfuscated kits. Moreover, due to author's re-utilization, our classifiers are able to signal even the kits that employ novel evasion and obfuscation techniques and that were not considered during training.

A large set of experiments investigate which ML models are the most suitable in which conditions. We can conclude that most ML classifiers guarantee good performance on the identification of evasive and obfuscated kits.
An interesting and initially unexpected outcome is that the results of the majority of the proposed classifiers are almost insensitive to the dimension of the dataset used in the training phase. More precisely, even training on just 20\% of the available phishing kits does not worsen much the results with respect to training experiments carried out on the typical 80\% of the dataset, despite a slight drop in the classification precision. 
%*** QUESTA PARTE E' RISCHIOSA: SI STA DICENDO CHE TUTTI I CLASSIFICATORI SONO BUONI E TUTTI SONO ROBUSTI PERCHE' FUNZIOANNO BENE CON IL 20\% DI TRAINING. POSSIBILE? SE SI', VA SPIEGATO MOLTO BENE PERCHE' SONO RISULTATI INATTESI E CONTROINTUITIVI. FORSE S IVOELVA DIRE ALTRO ***
Although we evaluate our method on a vast corpus of phishing kits, they represent a small fraction of existing and novel kits. Hence, the robustness of our results trained on small sets further demonstrates the effectiveness of our proposal in classifying even future new kits.

%*** QUESTA PARTE E' FONDAMENTALE ED E' SCRITTA MALE.

%1) SI ANTICIPA CHE NON SERVE PER LA DETECTION E POI SI DICE ESATTAMENTE IL CONTRARIO



%2) POI SI AGGIUNGE UN RISULTATO DI PROFILING MAI ACCENNATO IN PRECEDENZA. SE E' UN RISULTATO INTERESSANTE, VA CITATO PRIMA 



%*******************************

%PROBABILMENTE E' TUTTA QUESTA PARTE CHE VA ANTICIPATA PERCHE' OGNI LETTORE SI E' GIA' CHIESTO A COSA SERVIAMO. E NON PUO' SCOPRIRLO A PAGINA 4 ...

%*******************************

The remainder of this paper is organized as follows. Section \ref{sec:background} contains some background information about phishing kits and typical evasion and obfuscation techniques.
%Section \ref{sec:proposed_method} presents the different phases we follow to obtain the proposed classification. 
Section \ref{sec:classification} describes the three phases of our method. Section \ref{sec:deterministic} presents the results of the deterministic classification, while Section \ref{sec:ml_results}  details machine learning algorithms and considered scenarios. Section~\ref{sec:ml_evaluation} discusses the results of the probabilistic classification. Section \ref{sec:related} compares our work against related literature. Finally, Section \ref{sec:conclusions} draws conclusions and presents some possible extension of the results of this paper.




==> sections/old/2-background.tex <==
\section{Background and Motivation}
\label{sec:background}

Phishing is a criminal cyber attack belonging to the category of social engineering. It is designed to fool unwary victims by making them believe that they are interacting with a legitimate website, and inducing them to insert their credentials~\cite{das2019sok}. 
The popularity of this attack continues to grow, with thousands of new phishing URLs found every day. As an example, the Anti-Phishing Working Group reports more than $1\,000\,000$ phishing attacks just in the first quarter of 2022~\cite{apwg2022report}.
\textit{Spear} phishing is a dangerous variant directed towards the employees of a specific organization after an intelligence phase on the target~\cite{caputo2013going}. The false sense of security created by the alleged sender and proper subject increase the chances of success for an attacker~\cite{williams2018exploring, alsharnouby2015phishing}.

Phishing attacks consist of several phases where sending malicious emails is just one middle action~\cite{alabdan2020phishing}. The attackers need to initially implement and deploy a website mimicking that of the targeted organization. This site must be integrated with web forms to collect user credentials or other information. Only afterwards, attackers begin the phishing message campaign aimed to lure a large number of victims to their malicious website and induce them to insert their credentials.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Phishing kit business}
\label{sec:pk_business}

Phishing kits are created by expert attackers to automate the time-consuming and error-prone phases of implementation and deployment of a counterfeit copy of a legitimate website.
These kits consist of archives containing all the necessary components to deploy a fake website~\cite{bijmans2021catching}. In their basic version, they include server-side code implementing the logic of the website, along with several mimic web pages to induce the visitors to send their data. However, as detection systems improve, phishing kits evolve as well. Modern kits include novel and newly combined versions of evasion and obfuscation functions as countermeasures against anti-phishing tools (e.g.,~\cite{han2016phisheye, oest2018inside, cova2008there}), like in a typical cat-and-mouse game.
Through phishing kits, the phishers can rapidly obtain a working environment by uploading and extracting the content of a kit on an operational web server.  This facilitation is behind the amazing growth of phishing attacks in recent years. 
%The motivation of this paper comes from the observation that public cloud and host providers are quite interested to avoid being involved in similar criminal activities, as they risk IP banning and reputation issues.

Cyber crime is now a mature industry that is characterized by specializations together with markets for exchange and sale of products. Even phishing has reached the maturity of the \textit{Crime-as-a-Service} business model where expert cybercriminals sell or rent malicious products and services to third party actors that do not necessarily have strong technical skills. Nowadays, phishing kits represent a product of the \textit{Phishing-as-a-Service} business~\cite{chiew2018survey}. In Figure~\ref{fig:phaas} we outline a possible modern workflow. An expert author implements a phishing kit (step 1) and provides it to the phishers community through different business relationships (step 2). Each kit typically comes with a dedicated section in which an user can specify his preferred email addresses on which he wishes to receive the stolen credentials. Hence, once a phisher has bought a kit, it is sufficient that he adds his destination lists and that he uploads the kit on a controlled web server. He then extracts its content and begins the phishing email campaign (step 3). Finally, as a typical fisherman, he waits for victims to interact with the uploaded website (step 4) and collects the exfiltrated information (step 5).
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.3\columnwidth, center]{figures/schemas/PhaaS.pdf}
    \caption{Phishing-as-a-Service workflow.}
    \label{fig:phaas}
\end{figure*}
For the goal of this paper, it is important to observe that the authors of the phishing kits and their customers (\textit{phishers}) collaborate, but they typically belong to different groups. The community of expert authors is much smaller than that of the phisher customers because this business model facilitates even inexpert criminals to carry out sophisticated phishing attacks. 

As in any business model, the authors want to maximize their profits. This can be achieved through higher prices or by selling more products. The latter choice is more frequent, hence it can be expected that the phishing kit authors tend to re-use (even large) parts of their previous material, as confirmed also by other related works (e.g.,~\cite{bijmans2021catching, oest2018inside, merlo2022phishing}).
We leverage this hypothesis for the classification of the over 2000 analyzed phishing kits. As a second goal, we use machine learning algorithms as a way to extend the initial classification even to phishing kits that employ novel techniques that were not seen for training.

\subsection{Evasion techniques}
\label{sec:clas_evasion}

The anti-phishing environment continues to improve, but phishing kits are evolving as well. 
Evasion techniques represent one of the most important functions of the modern kits. They aim to elude detection of defensive tools~\cite{oest2019phishfarm} by preventing or delaying identification of phishing pages~\cite{zhang2021crawlphish}. An often adopted approach manipulates the \file{.htaccess} file in order to prevent access to unwanted visitors to the phishing page. This file is typically used as a legitimate access control filter in Apache Web servers, but it can be exploited by phishers to filter out network traffic coming from cybersecurity companies or from people of the target organization~\cite{han2016phisheye}. A similar filtering function is provided by the \file{robots.txt} file. It is typically used to give indications to automatic search engines regarding how to crawl a site, but it can also be configured to prevent access to automatic defensive tools. Attackers can also use filtering policies by implementing complex access control mechanisms into the logical level of their applications. For example, our exploratory analysis evidenced several sophisticated kits that record the IP addresses of their victims, and apply multiple mechanisms to redirect users to the page of the targeted organization. As phishing kits are built to remain unnoticed, a classification on the basis of the adopted evasion technique yields precious information about the phishing kit and author habits in writing malicious code.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obfuscation techniques}
\label{sec:clas_obfuscation}
Obfuscation techniques are used to conceal the original source code, thus complicating static analyses and reverse engineering investigations~\cite{you2010malware}. It is important to classify phishing kits according to the adopted obfuscation approach because there are several exploitable methods. 
Obfuscation can also be used to hide malicious functions (e.g., backdoors~\cite{cova2008there}), and to prevent intelligence about the real purposes of the phishers. Similarly to evasion techniques, there are multiple methods that authors can implement to obfuscate the source code of a phishing kit~\cite{proofpoint2016obfuscation}.
A typical obfuscation pattern adopts the PHP \codeword{eval} function, which dynamically evaluates and executes an obfuscated portion of the code. Some authors implement one-line coding or hex assignment strategies. Multiple automatic obfuscation tools (\textit{obfuscators}) are freely available online and are exploited in the wild. The classification of kits employing specific obfuscation techniques represent a relevant aspect to consider when developing automatic malicious code detection mechanisms.

==> sections/old/feat_table.tex <==
\begin{table}[ht!]
    \centering
    \caption{Feature set for the considered classifiers}
    \label{tab:feature_set}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|m{0.5cm}|c|c|c|}
            \hline
            % STRUCTURAL FEATURES
            \rowcolor[HTML]{EFEFEF} 
            \textbf{} & \textbf{Feature} & \textbf{Description} & \textbf{Type} \\ \hline \hline
             & \textit{nFiles} & Number of files & Numerical \\ \cline{2-4}
             & \textit{nDir} & Number of directories & Numerical\\ \cline{2-4}
             & \textit{nPhp} & Number of PHP files & Numerical \\ \cline{2-4}
             & \textit{nJs} & Number of Javascript files & Numerical \\ \cline{2-4}
             & \textit{nTxt} & Number of text files & Numerical \\ \cline{2-4}
             & \textit{nExe} & Number of Executables & Numerical\\ \cline{2-4}
             & \textit{nDll} & Number of dynamic-link libraries & Numerical \\ \cline{2-4}
             & \textit{nApk} & Number of Android Package files & Numerical \\ \cline{2-4}
             & \textit{nHtml} & Number of HTML files & Numerical \\ \cline{2-4}
             & \textit{nCss} & Number of CSS files & Numerical \\ \cline{2-4}
             & \textit{nPdf} & Number of PDF files & Numerical \\ \cline{2-4}
             & \textit{nMul} & Number of multimedia (images and videos) files & Numerical \\ \cline{2-4}
            \hspace{3pt}\multirow{-13}{*}{\rotatebox[origin=c]{90}{\textbf{Structural features}}} & \textit{Otherfiles} & Number of other files & Numerical \\ \hline \hline
            
            % RELEVANT FILES
             & \file{htaccess} & Presence of \file{.htaccess} file & Bool \\ \cline{2-4}
             & \file{robots.txt} & Presence of \file{robots.txt} file & Bool \\ \cline{2-4}
             & \textit{admin} & Presence of files or directories named "admin" & Bool \\ \cline{2-4}
            \hspace{5pt}\multirow{-4}{*}{\rotatebox[origin=c]{90}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Relevant \\ files \end{tabular}}}}} & \textit{config} & Presence of files or directories which contains "config" in name & Bool \\ \hline \hline
            
            % DEVELOPMENT FRAMEWORK
             & \textit{wordpress} & Use of Wordpress & Bool \\ \cline{2-4}
             & \textit{laravel} & Use of Laravel & Bool \\ \cline{2-4}
             & \textit{code\_ign} & Use of CodeIgniter & Bool \\ \cline{2-4}
             & \textit{zend} & Use of Zend & Bool \\ \cline{2-4}
            \hspace{4pt}\multirow{-5}{*}{\rotatebox[origin=c]{90}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Development \\ Frameworks \end{tabular}}}}} & \textit{HTTrack} & Use of website copier HTTrack & Bool \\ \hline \hline
            
            % PHP FUNCTIONS
             & \textit{api\_call} & Call to external API & Bool \\ \cline{2-4}
             & \textit{array\_hostnames} & Presence of array of hostnames & Bool \\ \cline{2-4}
             & \textit{array\_ipaddresses} & Presence of array of IP addresses & Bool \\ \cline{2-4}
             & \textit{form\_validation} & Form validation & Bool \\ \cline{2-4}
             & \textit{deceiving\_url} & Similarity between deployment url and target organization name & Bool \\ \cline{2-4}
             & \textit{deceiving\_zipname} & Similarity between zip name and target organization name & Bool \\ \cline{2-4}
             & \textit{read\_file} & Presence of \codeword{read} function call & Bool \\ \cline{2-4}
             & \textit{redirection} & Presence of redirection function & Bool \\ \cline{2-4}
             & \textit{random\_file} & Creation of randomly named files & Bool \\ \cline{2-4}
            \hspace{4pt}\multirow{-11}{*}{\rotatebox[origin=c]{90}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}PHP Functions \end{tabular}}}}} & \textit{random\_dir} & Creation of randomly named directories & Bool \\ \hline \hline
            
            % SUPERGLOBAL VARIABLES
             & \codeword{\$\_SERVER} & Use of \codeword{\$\_SERVER} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_GET} & Use of \codeword{\$\_GET} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_POST} & Use of \codeword{\$\_POST} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_FILES} & Use of \codeword{\$\_FILES} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_REQUEST} & Use of \codeword{\$\_REQUEST} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_SESSION} & Use of \codeword{\$\_SESSION} superglobal variable & Bool \\ \cline{2-4}
             & \codeword{\$\_ENV} & Use of \codeword{\$\_ENV} superglobal variable & Bool \\ \cline{2-4}
            \hspace{4pt}\multirow{-8}{*}{\rotatebox[origin=c]{90}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Supergobal variables \end{tabular}}}}} & \codeword{\$\_COOKIE} & Use of \codeword{\$\_COOKIE} superglobal variable & Bool \\ \hline \hline
            
            % EXFILTRATION METHOD
             & \textit{mail} & Presence of \codeword{mail} function call & Bool \\ \cline{2-4}
             & \textit{bot\_telegram} & Presence of Telegram Bot API & Bool \\ \cline{2-4}
            \hspace{4pt}\multirow{-3}{*}{\rotatebox[origin=c]{90}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Exf.\\ method\end{tabular}}}}} & \textit{write} & Presence of \codeword{write} function call & Bool \\ \hline
            
        \end{tabular}
    }
\end{table}
